Average sensitivity of the Knapsack Problem

In resource allocation, we often require that the output allocation of an algorithm is stable against input perturbation because frequent reallocation is costly and untrustworthy. Varma and Yoshida (SODA'21) formalized this requirement for algorithms as the notion of average sensitivity. Here, the average sensitivity of an algorithm on an input instance is, roughly speaking, the average size of the symmetric difference of the output for the instance and that for the instance with one item deleted, where the average is taken over the deleted item. In this work, we consider the average sensitivity of the knapsack problem, a representative example of a resource allocation problem. We first show a $(1-\epsilon)$-approximation algorithm for the knapsack problem with average sensitivity $O(\epsilon^{-1}\log \epsilon^{-1})$. Then, we complement this result by showing that any $(1-\epsilon)$-approximation algorithm has average sensitivity $\Omega(\epsilon^{-1})$. As an application of our algorithm, we consider the incremental knapsack problem in the random-order setting, where the goal is to maintain a good solution while items arrive one by one in a random order. Specifically, we show that for any $\epsilon > 0$, there exists a $(1-\epsilon)$-approximation algorithm with amortized recourse $O(\epsilon^{-1}\log \epsilon^{-1})$ and amortized update time $O(\log n+f_\epsilon)$, where $n$ is the total number of items and $f_\epsilon>0$ is a value depending on $\epsilon$.

==> differential.tex <==
\section{Relation between Average Sensitivity and Differential Privacy}\label{app:differential}

\emph{Differential privacy}, proposed by Dwork \emph{et al.}~\cite{dwork2006calibrating} is related to average sensitivity.
% The main idea is to guarantee the privacy protection by
For $\epsilon>0$ and $\delta>0$, an algorithm is \emph{$(\epsilon,\delta)$-differential private} if for any set $S$ and a pair of two inputs $V$ and its ``neighbor'' $V'$, we have
\begin{align*}
    \Pr[\mathcal{A}(V)\in S]\leq \exp(\epsilon)\Pr[\mathcal{A}(V')\in S]+\delta,
\end{align*}
where $\mathcal{A}(V)$ is the output distribution of the algorithm for the input $V$.
In the context of the knapsack problem, it is natural to regard that $V$ and  $V'$ are neighbors when $V'$ is obtained from $V$ by deleting one item (or vice versa).

It is known that $(\epsilon,\delta)$-differential privacy implies that the total variation distance between $\mathcal{A}(V)$ and $\mathcal{A}(V')$ is at most $\epsilon+\delta$~\cite{vadhan2017complexity}.
Here, the \emph{total variation distance} $\TV(\mathcal{S},\mathcal{S}')$ between two distributions $\mathcal{S},\mathcal{S}'$ is given by $
  \min_{\mathcal{D}} \E_{(S,S') \sim \mathcal{D}} 1_{S=S'}$,
where $1_P$ is the indicator of a predicate $P$, i.e., it is $1$ if $P$ holds and $0$ otherwise, and the minimum is taken over distributions of a pair of sets such that its marginal distributions on the first and second coordinates are equal to $\mathcal{S}$ and $\mathcal{S}'$, respectively. The total variation distance differs from the earth mover's distance in that we measure the distance of sets by the trivial zero-one distance, and not by the Hamming distance.

==> old/algo_old.tex <==
%!TEX root=./main.tex


\section{General Case}\label{subsec:general}
In this section, we show an algorithm for the knapsack problem with a constant average sensitivity.
The algorithm presented in this section assumes that we can compute the optimal solution of the knapsack problem and frequently use it as a subroutine.
We will address this issue and provide an FPTAS with a constant average sensitivity in Section~\ref{sec:fptas}.

\subsection{Technical Overview}
Let us first explain the intuition behind our algorithm (Algorithm~\ref{alg:knapsack}).
Let us fix a parameter $\epsilon > 0$.
An item is \emph{large} if its weight is at least $\epsilon$ and \emph{small} otherwise.
If all items are small, Algorithm~\ref{alg:smallknapsack} has high approximation ratio and constant average sensitivity, and we are done.
On the other hand, if all items are large, the optimal solution has constant average sensitivity because any feasible solution has cardinality at most $\epsilon^{-1}$.
We will combine these two observations to obtain an algorithm for the general case.

We can think of the following algorithm.
Let $L$ be the set of large items.
We first take a subset $R \subseteq L$ with $w(R) \leq 1$ that maximizes $v(R)+\OPT(V\setminus L, 1-w(R))$.
% Among the candidates $R$ of the set of the large items in the solution, i.e., $R\subseteq X$ such that $w(R)\leq 1$, we take the one with the largest value of $v(R)+\OPT(V\setminus X, 1-w(R))$.
Let $\mathrm{SMALL}(V\setminus L, 1-w(R))$ \ynote{name Algorithm 1 $\mathrm{SMALL}$ (you can use Procedure macro)}\snote{grammar wakaranai node horyuu} be the output of Algorithm~\ref{alg:smallknapsack} on the instance $(V\setminus L, 1-w(R))$ (with appropriate scaling of the weight).
Then, we output $R\cup \mathrm{SMALL}(V\setminus L, 1-w(R))$.

This algorithm has the following two issues.
\begin{enumerate}
\item If the choice of $R$ changes upon deleting an item, the value of $1-w(R)$ also changes, and hence the set of small items added to the output may dramatically change.
\item We cannot actually apply Algorithm~\ref{alg:smallknapsack} on the instance $(V\setminus L, 1-w(R))$ if $w(R)$ is close to $1$; there could be an item in $V\setminus L$ whose weight is too large against the weight limit $1-w(R)$.
\end{enumerate}

We consider the first issue.
We can consider the following two cases when the set $R$ changes after deleting an item $i$.
\begin{enumerate}
\item If we remove a large item, $R$ may be no longer the candidate because of $i\in R$.
\item If we remove a small item, the algorithm may choose different $R$ because the value $\OPT(V\setminus L, 1-w(R))$ decreases.
\end{enumerate}
To handle the first case (deleting large items), we restrict the number of candidate sets from which $R$ is selected to be constant, instead of selecting $R$ from all subsets of $L$ with $w(R)\leq 1$. Let $\mathcal{R}$ be the set of the candidates.
% that could be $R$ into constant, instead of choosing $R$ from
Then, there is a constant number of items $i$ such that $i\in R$ holds for some candidate $R\in \mathcal{R}$ because $|R|\leq \epsilon^{-1}$.
Therefore, by taking average over $i$, this case contributes the average sensitivity by a constant.
The restriction of the candidates is implemented by choosing at most one candidate from the sets $R$ with $w(R)\in \left[s\delta \OPT(V,1),(s+1)\delta \OPT(V,1)\right)$ for each integer $s$, where $\delta > 0$ is a constant (see Line~\ref{line:smallestweight} in Algorithm~\ref{alg:knapsack}).

To handle the second case (deleting small items), we ensure that the distribution of $R$ does not change much by a small decrease of $\OPT(V\setminus L, 1-w(R))$.
To this end, instead of taking $R$ as the one with maximum value of $v(R)+\OPT(V\setminus L, 1-w(R))$ among $R\in \mathcal{R}$, we apply the exponential mechanism~\cite{mcsherry2007mechanism}; we sample $R$ with probability proportional to the exponential of this value with appropriate scaling and rounding (see Line~\ref{line:exponential} on Algorithm~\ref{alg:knapsack}).
The scaling factor of the exponential mechanism should be proportional to the value $\OPT(V,1)$ \ynote{is this really proportional to $\OPT(V,1)$, not the sum of $v(R) +\OPT(V\setminus L, 1-w(R))$?}.
This implies that the scaling factor varies when some item is deleted, which is undesirable for the analysis sake.
%, we do not want the scaling factor changes by deleting an item. \ynote{what does this mean?}\snote{taiouzumi, Is it clear?}
To resolve this issue, we sample the scaling factor from an appropriately defined distribution so that it does not change much on average (see Line~\ref{line:choicec} of Algorithm~\ref{alg:knapsack}).
% to ensure that the removal of an item does not change the distribution of the denominator so much in average

Now, we consider the second issue. The main idea is to recursively apply the algorithm on the instance $(V\setminus L, 1-w(R))$ with appropriate scaling.
For each integer $r$, let $R_r$ be the set $R$ chosen in the $r$-th recursion step.
Let $K=\lceil \epsilon^{-1}\rceil$ be an integer.
Since the disjoint union of $R_1,\dots, R_K$ is a feasible solution of the instance $V$, the average of $v(R_1),\dots, v(R_K)$ is at most $\epsilon \OPT(V,1)$.
Therefore, if we sample an integer $k\in \{1,\dots, K\}$ uniformly at random, we can remove $R_k$ from the solution without deteriorating the approximation ratio much.
That means we can ignore all the large items in the $k$-th recursion step and apply Algorithm~\ref{alg:smallknapsack} (see Line~\ref{line:small} of Algorithm~\ref{alg:knapsack}).

Algorithm~\ref{alg:knapsack} has a parameter $\epsilon > 0$.
%In the algorithm, we use two integers $K :=\lceil \epsilon^{-1}\rceil$ and $l :=\lceil \epsilon^{-2}\rceil$ and a real number $C :=\epsilon^{3}$.
\ynote{should be written in the pseudocode}\snote{taiouzumi}
Without loss of generality, we can assume that $\epsilon\leq 0.01$.
We denote by $\mathrm{SMALL}(U, W)$ the output of Algorithm~\ref{alg:smallknapsack} applied on the instance with the item set $U$, where the weight of the all items are multiplied by $\frac{1}{W}$; the weights are scaled to set weight limit to be $1$.

Note that, $U_{k+1}=U_k\setminus L_k$ ensures the applicability of Algorithm~\ref{alg:smallknapsack} at Line~\ref{line:small} because all items with weight at least $\epsilon W_k$ are in $L_k$.

\begin{algorithm}[t!]
\caption{Less-sensitive Knapsack}
\begin{algorithmic}[1]\label{alg:knapsack}
\STATE $K :=\lceil \epsilon^{-1}\rceil$, $l := \lceil \epsilon^{-2}\rceil$, $C := \epsilon^{3}$
\STATE Let $W_0\leftarrow 1, U_0\leftarrow V$
\FOR{$r=0,\dots, K-1$}
    \STATE Let $L_r\subseteq U_r$ be the set of items with weight at least $\epsilon W_r$
    \FOR{$t=0,\dots, l$}
        \IF{there is a subset of $L_r$ with value in $\left[\frac{t}{l} \OPT(U_r,W_r),\frac{t+1}{l} \OPT(U_r,W_r)\right)$}
            \STATE Let $A_{r,t}\subseteq L_r$ be the set of items with smallest weight that satisfies $\frac{t}{l} \OPT(U_r,W_r) \leq v(A_{r,t}) < \frac{t+1}{l} \OPT(U_r,W_r)$\label{line:smallestweight}
            \STATE Let $x_{r,t}=\frac{t}{l} \OPT(U_r,W_r) + \OPT(U_r\setminus L_r, W_r-w(A_{r,t}))$\label{line:defx}
        \ELSE
            \STATE Let $A_{r,t}=\emptyset$ and $x_{r,t}=-\infty$
        \ENDIF
    \ENDFOR
    \STATE Sample $c_r$ from the uniform distribution over $[C\cdot \OPT(U_r,W_r),2C\cdot \OPT(U_r,W_r)]$\label{line:choicec}
    \STATE Sample $t^{\circ}$ with probability proportional to $\exp(x_{r,t^{\circ}}/c_r)$\label{line:exponential}
    \STATE $R_{r+1} \leftarrow A_{r,t^{\circ}}$, $W_{r+1} \leftarrow W_r-w(R_{r+1})$, $U_{r+1} \leftarrow U_r\setminus L_r$
\ENDFOR
\STATE Choose an integer $k$ from the uniform distribution over $\{0,\dots, K-1\}$
\STATE Let $L_k\subseteq U_k$ be the set of items with weight at least $\epsilon W_k$
\RETURN $R_1\cup \dots \cup R_k \cup \mathrm{SMALL}(U_{k+1}, W_k)$\label{line:small}
\end{algorithmic}
\end{algorithm}


\subsubsection{Approximation Ratio}\label{subsec:approximation-ratio}

First, we analyze the approximation ratio.
% Let us fix an integer $r$, the set $U_r$ and the current weight limit $W_r$.
Consider the $r$-th iteration, and let $S^*_r$ be the set of items that attains $\OPT(U_r,W_r)$. Let $t^* \geq 0$ be an integer such that $v(S^*_r\cap L_r)\in \left[\frac{t^*}{l}\OPT(U_r,W_r),\frac{t^*+1}{l}\OPT(U_r,W_r)\right)$.

The following lemma bounds the loss in the approximation ratio caused by limiting the candidates of the chosen items in $L_r$ to $A_{r,0},\dots, A_{r,l}$.

\begin{lemma}\label{lem:errort}
It holds that
\begin{align}
    x_{r,t^*}\geq \left(1-2\epsilon^{2}\right)\OPT(U_r,W_r).
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    x_{r,t^*}&=\frac{t^*}{l}\OPT(U_r,W_r)+\OPT(U_r\setminus L_r, W-w(A_{r,t^*}))\\
    &\geq \frac{t^*}{l}\OPT(U_r,W_r)+\OPT(U_r\setminus L_r, W-w(S^*_r\cap L_r))\\
    &= \frac{t^*}{l}\OPT(U_r,W_r)+v(S^*_r\setminus L_r)\\
    &\geq v(S^*_r\cap L_r)-\frac{1}{l}\OPT(U_r,W_r)+v(S^*_r\setminus L_r)\\
    &=\left(1-\frac{1}{l}\right)\OPT(U_r,W_r)\\
    &\geq (1-2\epsilon^{2})\OPT(U_r,W_r),
\end{align}
where the first line is from the definition of $x_{r,t^*}$, the second line is from $w(A_{r,t^*})\leq w(S^*_r\cap L_r)$ that is ensured by Line~\ref{line:smallestweight} in the algorithm, the third line is from the optimality of $S^*_r$, the fourth line is from the definition of $t^*$, the fifth line is from the definition of $S^*_r$, and the last line is from $l=\lceil \epsilon^{-2}\rceil$ and $\epsilon\leq 0.01$.
\end{proof}

Next we analyze the loss in the approximation ratio caused by the exponential method. We prove the following.

\begin{lemma}\label{lem:errorexp}
$\E[x_{r,t^{\circ}}]\geq (1-2\epsilon^2) x_{r,t^*}$ holds.
\end{lemma}
\begin{proof}
Let $\gamma > 0$ be determined later. Then, we have
\begin{align}
    \Pr[x_{r,t^{\circ}}\leq (1-\gamma)x_{r,t^*}]
    &= \frac{\sum_{t\in \{0,\dots, l\}, x_{r,t}\leq (1-\gamma)x_{r,t^*}}\exp\left(\frac{x_{r,t}}{c_r}\right)}{\sum_{t\in \{0,\dots, l\}}\exp\left(\frac{x_{r,t}}{c_r}\right)}\\
    &\leq \frac{(l+1) \exp\left(\frac{(1-\gamma)x_{r,t^*}}{c_r}\right)}{\exp\left(\frac{x_{r,t^*}}{c_r}\right)}\\
    &= (l+1) \exp\left(- \frac{\gamma x_{r,t^*}}{c_r}\right)\\
    &\leq (l+1) \exp\left(- \frac{\gamma(1-2\epsilon^{2})\OPT(U_r,W_r)}{c_r}\right)\\
    &\leq (l+1) \exp\left(-\frac{\gamma(1-2\epsilon^{2})}{2C}\right).\label{eq:2c2c}
\end{align}
Here, the first line is from Line~\ref{line:exponential} of the algorithm, the second line is from the fact that there are at most $l+1$ indices $t$ with $x_{r,t}\leq (1-\gamma)x_{r,t^*}$, the fourth line is from Lemma~\ref{lem:errort}, and the last line is from $c_r\leq 2C\cdot \OPT(U_r,W_r)$.

Now, we set $\gamma=\epsilon^{2}$. Then, we have
\begin{align}
    \E[x_{r,t^{\circ}}]
    &\geq (1-\gamma)x_{r,t^*}\Pr[x_{r,t^{\circ}} > (1-\gamma)x_{r,t^*}]\\
    &\geq (1-\gamma) \left(1-(l+1)\exp\left(-\frac{\gamma(1-2\epsilon^{2})}{2C}\right)\right)x_{r,t^*}\\
    &= \left(1-\epsilon^{2}\right) \left(1-(\lceil \epsilon^{-2}\rceil +1)\exp\left(-\frac{\epsilon^{-1}(1-2\epsilon^{2})}{2}\right)\right)x_{r,t^*}\\
    &\geq (1-\epsilon^{2})^2 x_{r,t^*}\geq (1-2\epsilon^{2})x_{r,t^*}.
\end{align}
Here, the second line is from~\eqref{eq:2c2c}, the third line is from the definitions of $\gamma$, $l$ and $C$, the third line is from $\epsilon\leq 0.01$.

\end{proof}

Combining these results yields the following.

\begin{lemma}\label{lem:stepapprox}
$\E[v(R_{r+1})+\OPT(U_{r+1},W_{r+1})]\geq (1-4\epsilon^{2}) \OPT(U_r,W_r)$ holds.
\end{lemma}
\begin{proof}
We have
\begin{align}
    \E[v(R_{r+1})+\OPT(U_{r+1},W_{r+1})]
    &\geq \E[x_{r,t^{\circ}}]\\
    &\geq (1-2\epsilon^{2})x_{r,t^*}\\
    &\geq (1-2\epsilon^{2})^2\OPT(U_r,W_r)\\
    &\geq (1-4\epsilon^{2}) \OPT(U_r,W_r)
\end{align}
where the first line is from the Line~\ref{line:defx} of the algorithm, the second line is from Lemma~\ref{lem:errorexp}, and the last line is from Lemma~\ref{lem:errort}.
\end{proof}

Now we bound the approximation ratio of Algorithm~\ref{alg:knapsack}. Let $\mathcal{A}$ be the output distribution of Algorithm~\ref{alg:knapsack} on the instance $V$.

\begin{lemma}\label{lem:largeapprox}
The approximation ratio of Algorithm~\ref{alg:knapsack} is at least $1-8\epsilon$.
\end{lemma}
\begin{proof}
First, we prove
\begin{align}
    \E\left[\sum_{r=1}^k v(R_r) + \OPT(U_k,W_k)\right]\geq (1-4k\epsilon^2) \OPT(V,1)
\end{align}
by induction on $k$.
When $k=0$, the claim is clear from $U_0=V$ and $W_0=1$.
For $k\geq 1$, we can use Lemma~\ref{lem:stepapprox} to obtain
\begin{align}
    \E\left[\sum_{r=1}^k v(R_r) + \OPT(U_k,W_k)\right]
    &=\E\left[\sum_{r=1}^{k-1} v(R_r)\right] + \E[v(R_k) + \OPT(U_k,W_k)]\\
    &\geq \E\left[\sum_{r=1}^{k-1} v(R_r)\right] + (1-4\epsilon^2)\E[\OPT(U_{k-1},W_{k-1})]\\
    &\geq (1-4\epsilon^2)\E\left[\sum_{r=1}^{k-1} v(R_r) + \OPT(U_{k-1},W_{k-1})\right]\\
    &\geq (1-4\epsilon^2)(1-4(k-1)\epsilon^2) \OPT(V,1)\\
    &\geq (1-4k\epsilon^2) \OPT(V,1).\label{eq:4ke2}
\end{align}

Now, we have
\begin{align}
    \E[v(\mathcal{A})]
    &=\frac{1}{K}\sum_{k=0}^{K-1}\E\left[v\left(R_1\cup\dots\cup R_k\cup \mathrm{SMALL}(U_{k+1},W_k) \right)\right]\\
    &\geq \frac{1}{K}\sum_{k=0}^{K-1}\E\left[\sum_{r=1}^{k} v(R_r) + (1-2\epsilon) \OPT(U_{k+1},W_k)\right]\\
    &\geq \frac{1-2\epsilon}{K}\sum_{k=0}^{K-1}\E\left[\sum_{r=1}^{k} v(R_r) +  \OPT(U_{k+1},W_k)\right]\\
    &\geq \frac{1-2\epsilon}{K}\sum_{k=0}^{K-1}\E\left[\sum_{r=1}^{k} v(R_r) + \OPT(U_{k+1},W_{k+1})\right]\\
    &\geq \frac{1-2\epsilon}{K}\sum_{k=0}^{K-1}\E\left[\sum_{r=1}^{k} v(R_r) + \sum_{r=k+2}^{K} v(R_r) + \OPT(U_K,W_K)\right]\\
    &\geq \frac{1-2\epsilon}{K}\E\left[(K-1)\sum_{r=1}^{K} v(R_r) + K\OPT(U_K,W_K)\right]\\
    &\geq (1 - 2\epsilon)\left(1-\frac{1}{K}\right)\E\left[\sum_{r=1}^{K}v(R_r) + \OPT(U_K,W_K)\right]\\
    &\geq (1 - 2\epsilon)\left(1 - \frac{1}{K}\right)(1 - 4K\epsilon^2) \OPT(V,1)\\
    &\geq (1-2\epsilon)(1-\epsilon)(1-5\epsilon) \OPT(V,1)\\
    &\geq (1-8\epsilon) \OPT(V,1).
\end{align}
Here, the first line is from Line~\ref{line:small} in Algorithm~\ref{alg:knapsack}, the second line is from Lemma~\ref{lem:smallapprox}, the fourth line is from $W_k\geq W_{k+1}$, the fifth line is from the fact that the union of $R_{k+2}\cup \dots \cup R_K$ and the set that attains $\OPT(U_K,W_K)$ is a feasible solution of the knapsack problem on item set $U_{k+1}$ and weight limit $W_{k+1}$, the eighth line is from~\eqref{eq:4ke2}, and the ninth line is from $K=\lceil \epsilon^{-1}\rceil$ and $\epsilon\leq 0.01$.
\end{proof}




\subsubsection{Average Sensitivity}\label{subsec:sensitivity}

In this section, we bound the average sensitivity.

For $i \in V$, we denote by $R^i_1,\dots, R^i_{K}$ the sets $R_1,\dots, R_{K}$ used in the algorithm when the instance $V \setminus \{i\}$ so that the instance of interest is clear.
% Let $i\in V$ and consider running Algorithm~\ref{alg:knapsack} on the instance $V\setminus \{i\}$.
% denote the sets  run on $V \setminus \{i\}$.
% We simply denote the sets $R_1,\dots, R_K$ in Algorithm~\ref{alg:knapsack} on the instance $V$ by $R_1,\dots, R_K$.
Similarly, we define $U_r$, $U^i_r$, $W_r$, and $W^i_{r}$ for $r=0,\dots, K$, define $L_r$, $L^i_r$, $c_r$, and $c^i_r$ for $r=0,\dots, K-1$, and define $A_{r,t}$, $A^i_{r,t}$, $x_{r,t}$, and $x^i_{r,t}$ for $r=0,\dots, K-1$ and $t=0,\dots, l$.

We first prove that the distributions of the sequences $(R_1,\dots, R_K)$ and $(R^i_1,\dots, R^i_K)$ are sufficiently similar on average, where the average is taken over $i\in V$ (Lemma~\ref{lem:combined2}). After that, we combine the analysis for large items and small items (Lemma~\ref{lem:largesensitivity}). 
\ynote{I think having an overview of the proof here is helpful.}\snote{taiouzumi}

To prove Lemma~\ref{lem:combined2} by induction, suppose $R_1=R^i_1,\dots, R_r=R^i_r$ for some $r\in \{0,\dots, K-1\}$.
It follows that $U^i_r=U_r\setminus \{i\}$ and $W^i_r=W_r$ from the definition of the algorithm.
The objective here is to prove that the distribution of $R^i_{r+1}$ is sufficiently close to that of $R_{r+1}$ on average.
More specifically, we analyze the following quantity:
\begin{align}
    \sum_{i\in V}\sum_{A\subseteq V}\max\left(0,\Pr[R_{r+1}=A]-\Pr[R^i_{r+1}=A]\right).\label{eq:befdiffs}
\end{align}
Since $\Pr[R_{r+1}=A]$ is positive only if $A=A_{r,t}$ for some $t\in \{0,\dots, l\}$, we have
\begin{align}
    \eqref{eq:befdiffs} = \sum_{i\in V}\sum_{t\in \{0,\dots, l\}}\max\left(0,\Pr[R_{r+1}=A_{r,t}]-\Pr[R^i_{r+1}=A_{r,t}]\right).\label{eq:diffs}
\end{align}
%Furthermore, if $\OPT(U_r,W_r)\leq 2\OPT(U^i_r,W^i_r)$, we have
%\begin{align}
%    &\Pr[R_{r+1}=A_{r,t}]-\Pr[R^i_{r+1}=A_{r,t}]\\
%    &=\frac{1}{C\cdot \OPT(U_r,W_r)}\int_{C\cdot \OPT(U_r,W_r)}^{2C\cdot \OPT(U_r,W_r)}\Pr[R_{r+1}=A_{r,t}|c_r=c]\mathrm{d}c\\
%    &-\frac{1}{C\cdot \OPT(U^i_r,W^i_r)}\int_{C\cdot \OPT(U^i_r,W^i_r)}^{2C\cdot \OPT(U^i_r,W^i_r)}\Pr[R^i_{r+1}=A_{r,t}|c^i_r=c]\mathrm{d}c\\
%    &\leq \frac{1}{C\cdot \OPT(U_r,W_r)}\int_{C\cdot \OPT(U_r,W_r)}^{2C\cdot \OPT(U^i_r,W^i_r)}\left(\Pr[R_{r+1}=A_{r,t}|c_r=c]-\Pr[R^i_{r+1}=A_{r,t}|c^i_r=c]\right)\mathrm{d}c\\
%    &+\frac{2(\OPT(U_r,W_r)-\OPT(U^i_r,W^i_r))}{\OPT(U_r,W_r)},
%\end{align}
%here the equality is from the algorithm and inequality is from $\OPT(U^i_r,W^i_r)\leq \OPT(U_r,W_r)$ and $\Pr[R_{r+1}=A_{r,t}]-\Pr[R^i_{r+1}=A_{r,t}]\leq 1$.
%If $\OPT(U_r,W_r) > 2\OPT(U^i_r,W^i_r)$, we use the trivial bound $\Pr[R_{r+1}=A_{r,t}]-\Pr[R^i_{r+1}=A_{r,t}]\leq 1$.
We first bound~\eqref{eq:diffs} conditioned on that the values of $c_r$ and  $c^i_r$ are the same.
We consider the following three cases: $i\not \in U_r$, $i\in L_r$ and $i\in U_r\setminus L_r$.
% We fix the real number $c$ and analyze in a way that the case $c=c^i_r$ corresponds to the case $c=c_r$.
% Note that, $c^i_r$ and $c_r$ may have different distributions in general.

The next lemma handles the case $i\not \in U_r$.
\begin{lemma}\label{lem:baai1}
Let $c$ be a real number. Then,
\begin{align}
    \sum_{i\in V\setminus U_r}\sum_{t\in \{0,\dots, l\}}\max\left(0,\Pr[R_{r+1}=A_{r,t} \mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t} \mid c^i_r=c]\right)=0.
\end{align}
\end{lemma}
\begin{proof}
In this case, $R_{r+1}$ and $R^i_{r+1}$ are taken from the same distribution.
\end{proof}

The next lemma handles the case $i\in L_r$.
\begin{lemma}\label{lem:baai2}
Let $c$ be a real number. Then,
\begin{align}
    \sum_{i\in L_r}\sum_{t\in \{0,\dots, l\}}\max\left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\leq 2\epsilon^{-3}.
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    &\sum_{i\in L_r}\sum_{t\in \{0,\dots, l\}}\max\left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\\
    &= \sum_{i\in L_r}\sum_{t: i\not \in A_{r,t}}\max\left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\label{eq:notin}\\
    &+ \sum_{i\in L_r}\sum_{t: i\in A_{r,t}}\max\left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\label{eq:in}.
\end{align}

Let us fix $i\in L_r$ and $t\in \{0,\dots, l\}$, and assume $x_{r,t}\neq -\infty$. If $i\not \in A_{r,t}$, then we have
\begin{align}
    x_{r,t}&=\frac{t}{l}\OPT(U_r,W_r)+\OPT(U_r\setminus L_r,W_r-w(A_{r,t}))\\
    &=\frac{t}{l}\OPT(U^i_r,W^i_r)+\OPT(U^i_r\setminus L^i_r,W^i_r-w(A_{r,t}))\\
    &=\frac{t}{l}\OPT(U^i_r,W^i_r)+\OPT(U^i_r\setminus L^i_r,W^i_r-w(A^i_{r,t}))=x^i_{r,t},\label{line:xeqx}
\end{align}
where the second equality is from $i\in L_r$ and the third equality is from $A_{r,t}=A^i_{r,t}$ due to the definitions of $A_{r,t}$ and $A^i_{r,t}$.
If $i\in A_{r,t}$, then we have
\begin{align}
    x_{r,t}
    &= \frac{t}{l}\OPT(U_r,W_r)+\OPT(U_r\setminus L_r,W_r-w(A_{r,t}))\\
    &= \frac{t}{l}\OPT(U^i_r,W^i_r)+\OPT(U^i_r\setminus L^i_r,W^i_r-w(A_{r,t}))\\
    &\geq \frac{t}{l}\OPT(U^i_r,W^i_r)+\OPT(U^i_r\setminus L^i_r,W^i_r-w(A^i_{r,t}))=x^i_{r,t},\label{line:xgeqx}
\end{align}
where the second equality is from $i\in L_r$ and the inequality is from $w(A_{r,t})\leq w(A^i_{r,t})$ that follows from Line~\ref{line:smallestweight} of Algorithm~\ref{alg:knapsack}.

If $x^i_{r,t}=-\infty$, the inequality $x_{r,t}\geq x^i_{r,t}$ trivially holds. Therefore, for all $t\in \{0,\dots, l\}$ and $i\in L_r$ we have $x_{r,t}\geq x^i_{r,t}$.

Now, for $t\in \{0,\dots, l\}$ and $i\not \in A_{r,t}$, we have
\begin{align}
    \Pr[R_{r+1}=A_{r,t}\mid c_r=c] &= \frac{\exp(x_{r,t}/c)}{\sum_{t'\in \{0,\dots, l\}}\exp(x_{r,t'}/c)}\\
    &= \frac{\exp(x^i_{r,t}/c)}{\sum_{t'\in \{0,\dots, l\}}\exp(x_{r,t'}/c)}\\
    &\leq \frac{\exp(x^i_{r,t}/c)}{\sum_{t'\in \{0,\dots, l\}}\exp(x^i_{r,t'}/c)}=\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c].
\end{align}
Here, the first and the last equality is from Line~\ref{line:exponential} of Algorithm~\ref{alg:knapsack}, the second equality is from~\eqref{line:xeqx}, the inequality is from $x_{r,t'}\geq x^i_{r,t'}$.
Therefore the value of~\eqref{eq:notin} is zero.


Now we evaluate~\eqref{eq:in}. We have
\begin{align}
    \eqref{eq:in}
    &\leq \sum_{i\in L_r}\sum_{t:i\in A_{r,t}}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\leq \sum_{t\in \{0,\dots, l\}}|A_{r,t}|\leq (l+1)\epsilon^{-1}\leq 2\epsilon^{-3},
\end{align}
where the second inequality is from $\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\leq 1$, the third inequality is from $|A_{r,t}|\leq \epsilon^{-1}$, and the last inequality is from $l=\lceil \epsilon^{-2}\rceil$ and $\epsilon\leq 0.01$.
Therefore the lemma is proved.
\end{proof}

Now we consider the case $i\in U_r\setminus L_r$. The following lemma is elementary.
\begin{lemma}\label{lem:diffsum}
For any item set $U$ and weight limit $W$, we have
\begin{align}
    \sum_{i\in U}(\OPT(U,W)-\OPT(U\setminus \{i\},W))\leq \OPT(U,W).
\end{align}
\end{lemma}
\begin{proof}
Let $S$ be the optimal solution of the instance $(U,W)$. If $i\not \in S$, we have $\OPT(U,W)=\OPT(U\setminus \{i\},W)$ because $S$ is still a feasible solution of the instance $(U\setminus \{i\},W)$. If $i\in S$, we have $\OPT(U\setminus \{i\},W)\geq \OPT(U,W)-v(i)$ because $S\setminus \{i\}$ is a feasible solution of the instance $(U\setminus \{i\},W)$. Therefore, we have
\begin{align}
    \sum_{i\in U}(\OPT(U,W)-\OPT(U\setminus \{i\},W))
    \leq \sum_{i\in S}v(i) = \OPT(U,W).
\end{align}
\end{proof}

Now we prove the following lemma.
\begin{lemma}\label{lem:baai3}
Let $c$ be a real number. Then,
\begin{align}
    \sum_{i\in U_r\setminus L_r}\sum_{t\in \{0,\dots, l\}}\max\left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\leq \epsilon^{-3}.
\end{align}
\end{lemma}
\begin{proof}
Let us fix $i\in U_r\setminus L_r$ and $t\in \{0,\dots, l\}$, and assume $x_{r,t}\neq -\infty$. Then, we have
\begin{align}
    x_{r,t}&=\frac{t}{l}\OPT(U_r,W_r)+\OPT(U_r\setminus L_r,W_r-w(A_{r,t}))\\
    &= \frac{t}{l}\OPT(U^i_r,W^i_r)+\OPT((U^i_r\setminus L^i_r)\cup \{i\} ,W^i_r-w(A_{r,t}))\\
    &= \frac{t}{l}\OPT(U^i_r,W^i_r)+\OPT((U^i_r\setminus L^i_r)\cup \{i\} ,W^i_r-w(A^i_{r,t}))\\
    &\geq \frac{t}{l}\OPT(U^i_r,W^i_r)+\OPT(U^i_r\setminus L^i_r ,W^i_r-w(A^i_{r,t}))=x^i_{r,t},\label{eq:xgggeqx}
\end{align}
where the second equality is from $i\in U_r\setminus L_r$, the third equality is because $L_r=L^i_r$ and hence $A_{r,t}=A^i_{r,t}$.
Therefore, we have
\begin{align}
    &\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\\
    &= \frac{\exp(x_{r,t}/c)}{\sum_{t\in \{0,\dots, l\}}\exp(x_{r,t}/c)} - \frac{\exp(x^i_{r,t}/c)}{\sum_{t\in \{0,\dots, l\}}\exp(x^i_{r,t}/c)}\\
    &\leq \frac{\exp(x_{r,t}/c)-\exp(x^i_{r,t}/c)}{\sum_{t\in \{0,\dots, l\}}\exp(x_{r,t}/c)}\\
    &= \left(1-\exp\left(-\frac{x_{r,t}-x^i_{r,t}}{c}\right)\right)\frac{\exp(x_{r,t}/c)}{\sum_{t\in \{0,\dots, l\}}\exp(x_{r,t}/c)}\\
    &\leq \frac{x_{r,t}-x^i_{r,t}}{c}\Pr[R_{r+1}=A_{r,t}\mid c_r=c].\label{eq:explinear}
\end{align}
Here, the second line is from Line~\ref{line:exponential} of Algorithm~\ref{alg:knapsack}, the third line is from~\eqref{eq:xgggeqx}, and the last line is from $1-\exp(-x)\leq x$.
Now, we have
\begin{align}
    &\sum_{i\in U_r\setminus L_r}\sum_{t\in \{0,\dots, l\}}\max\left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\\
    &\leq \sum_{i\in U_r\setminus L_r}\sum_{t\in \{0,\dots, l\}}\frac{x_{r,t}-x^i_{r,t}}{c}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\\
    &\leq \frac{\OPT(U_r\setminus L_r,W_r-w(A_{r,t}))}{c}\sum_{t\in \{0,\dots, l\}}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\\
    &\leq \frac{\OPT(U_r,W_r)}{c}\sum_{t\in \{0,\dots, l\}}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\\
    &\leq \frac{1}{C} = \epsilon^{-3}.
\end{align}
Here, the first inequality is from~\eqref{eq:xgggeqx} and~\eqref{eq:explinear}. The second inequality is from
\begin{align}
    &\sum_{i\in U_r\setminus L_r}(x_{r,t}-x^i_{r,t})\\
    &=\sum_{i\in U_r\setminus L_r}(\OPT(U_r\setminus L_r,W_r-w(A_{r,t}))-\OPT((U_r\setminus L_r)\setminus \{i\},W_r-w(A_{r,t})))\\
    &\leq \OPT(U_r\setminus L_r,W_r-w(A_{r,t})),
\end{align}
which is obtained from Lemma~\ref{lem:diffsum}. The last inequality is from Line~\ref{line:choicec} of Algorithm~\ref{alg:knapsack}.
\end{proof}

Combining Lemmas~\ref{lem:baai1},~\ref{lem:baai2}, and~\ref{lem:baai3} yields the following.
\begin{lemma}\label{lem:combined}
We have
\begin{align}
    \sum_{i\in V}\sum_{t\in \{0,\dots, l\}}\max \left(0, \Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\leq 3\epsilon^{-3}.
\end{align}
\end{lemma}
\begin{proof}
This immediately follows from Lemma~\ref{lem:baai1},~\ref{lem:baai2} and~\ref{lem:baai3} the fact that $V$ is a disjoint union of $V\setminus U_r$, $L_r$ and $U_r\setminus L_r$.
\end{proof}

Now we bound the difference between the distributions of $R_{r+1}$ and $R^i_{r+1}$ unconditioning the assumption that $c_r$ and $c_r^i$ are the same.

\begin{lemma}\label{lem:combined1.5}
We have
\begin{align}
    \sum_{i\in V}\sum_{A\subseteq V}\max\left(0,\Pr[R_{r+1}=A]-\Pr[R^i_{r+1}=A]\right)\leq 4\epsilon^{-3}.
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    &\max \left(0,\Pr[R_{r+1}=A_{r,t}]-\Pr[R^i_{r+1}=A_{r,t}]\right)\\
    &=\max \left(0,\frac{1}{C\cdot \OPT(U_r,W_r)}\int_{C\cdot \OPT(U_r,W_r)}^{2C\cdot \OPT(U_r,W_r)}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\mathrm{d}c \right.\nonumber \\
    &\left.\quad \quad \quad \quad -\frac{1}{C\cdot \OPT(U^i_r,W^i_r)}\int_{C\cdot \OPT(U^i_r,W^i_r)}^{2C\cdot \OPT(U^i_r,W^i_r)}\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\mathrm{d}c \right)\\
    &\leq \frac{1}{C\cdot \OPT(U_r,W_r)}\left(\int_{2C\cdot \OPT(U^i_r,W^i_r)}^{2C\cdot \OPT(U_r,W_r)}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\mathrm{d}c\right.\nonumber \\
    & \: \left.+\int_{C\cdot \OPT(U_r,W_r)}^{2C\cdot \OPT(U^i_r,W^i_r)}\max \left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\mathrm{d}c\right),\label{eq:dividecc}
\end{align}
where the equality is from Line~\ref{line:choicec} of Algorithm~\ref{alg:knapsack} and the inequality is from the triangle inequality and
\begin{align}
    \frac{1}{C\cdot \OPT(U_r,W_r)}\leq \frac{1}{C\cdot \OPT(U^i_r,W^i_r)},
\end{align}
which follows from $\OPT(U_r,W_r)\geq \OPT(U^i_r,W^i_r)$.

Now, we have
\begin{align}
    &\sum_{i\in V}\sum_{t\in \{0,\dots, l\}}\frac{1}{C\cdot \OPT(U_r,W_r)}\int_{2C\cdot \OPT(U^i_r,W^i_r)}^{2C\cdot \OPT(U_r,W_r)}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\mathrm{d}c\\
    &\leq \sum_{t\in \{0,\dots, l\}}\frac{1}{C\cdot \OPT(U_r,W_r)}\sum_{i\in V}\left(2C\cdot (\OPT(U_r,W_r)-\OPT(U^i_r,W^i_r))\right)\\
    &\leq \sum_{t\in \{0,\dots, l\}}\left(\frac{1}{C\cdot \OPT(U_r,W_r)}\cdot 2C\cdot \OPT(U_r,W_r)\right) = 2(l+1) \leq 3\epsilon^{-2},\label{eq:3e2}
\end{align}
where the first inequality is from $\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\leq 1$, the second inequality is from Lemma~\ref{lem:diffsum}, and the last inequality is from $l=\lceil \epsilon^{-2} \rceil$ and $\epsilon\leq 0.01$.

Therefore, we have
\begin{align}
    &\sum_{i\in V}\sum_{A\subseteq V}\max\left(0,\Pr[R_{r+1}=A]-\Pr[R^i_{r+1}=A]\right)\\
    &= \sum_{i\in V}\sum_{t\in \{0,\dots, l\}}\max\left(0,\Pr[R_{r+1}=A_{r,t}]-\Pr[R^i_{r+1}=A_{r,t}]\right)\\
    &\leq \sum_{i\in V}\sum_{t\in \{0,\dots, l\}}\frac{1}{C\cdot \OPT(U_r,W_r)}\left(\int_{2C\cdot \OPT(U^i_r,W^i_r)}^{2C\cdot \OPT(U_r,W_r)}\Pr[R_{r+1}=A_{r,t}\mid c_r=c]\mathrm{d}c\right.\nonumber \\
    & \: \left.+\int_{C\cdot \OPT(U_r,W_r)}^{2C\cdot \OPT(U^i_r,W^i_r)}\max \left(0,\Pr[R_{r+1}=A_{r,t}\mid c_r=c]-\Pr[R^i_{r+1}=A_{r,t}\mid c^i_r=c]\right)\mathrm{d}c\right)\\
    &\leq 3\epsilon^{-2} + \frac{1}{C\cdot \OPT(U_r,W_r)}\int_{C\cdot \OPT(U_r,W_r)}^{2C\cdot \OPT(U^i_r,W^i_r)}3\epsilon^{-3}\mathrm{d}c\\
    &\leq 3\epsilon^{-2} + \frac{1}{C\cdot \OPT(U_r,W_r)}\cdot 3\epsilon^{-3}\cdot C\cdot \OPT(U_r,W_r)\\
    &= 3\epsilon^{-2}+3\epsilon^{-3}\leq 4\epsilon^{-3},
\end{align}
where the first inequality is from~\eqref{eq:dividecc}, the second inequality is from~\eqref{eq:3e2} and Lemma~\ref{lem:combined}, the third inequality is from $\OPT(U^i_r,W^i_r)\leq \OPT(U_r,W_r)$, and the last inequality is from $\epsilon \leq 0.01$.
\end{proof}

Now, we prove that the distribution of the sequence $(R^i_1,\dots, R^i_K)$ is close to that of the sequence $(R_1,\dots, R_K)$ on average.
For $k=0,\dots, K$, let $\mathcal{P}(A_1,\dots, A_k)$ (resp., $\mathcal{P}^i(A_1,\dots, A_k)$) be the event $R_1=A_1\land \dots \land R_k=A_k$ (resp., $R^i_1=A_1\land \dots \land R^i_k=A_k$).
First, we prove the following technical lemma.
\begin{lemma}\label{lem:tech}
Let $a,b,\alpha,\beta$ be non-negative numbers. Then, we have
\begin{align*}
    \max(0,a\alpha-b\beta) \leq a\max(0,\alpha-\beta)+\alpha \max(0,a-b).
\end{align*}
\end{lemma}
\begin{proof}
If $a\alpha-b\beta < 0$, then the statement is clear.
Hence in what follows, we assume $a\alpha \geq b\beta$ and specifically, $a\geq b$ or $\alpha \geq \beta$. From symmetry of $(a,b)$ and $(\alpha,\beta)$, we can assume $a\geq b$ \ynote{as $a\alpha \geq b\beta$ is not symmetric with respect to $a$ and $b$, I'm not sure this is wlog.}\snote{teineini shita}.

If $\alpha\geq \beta$, then we have
\begin{align}
    \max(0,a\alpha-b\beta)
    &=a\alpha-b\beta\\
    &=a(\alpha-\beta)+\alpha(a-b)-(a-b)(\alpha-\beta)\\
    &\leq a(\alpha-\beta)+\alpha(a-b)\\
    &=a\max(0,\alpha-\beta)+\alpha \max(0,a-b).
\end{align}
If $\alpha < \beta$, then we have
\begin{align}
    \max(0,a\alpha-b\beta)
    &=a\alpha-b\beta\\
    &=\alpha(a-b)-b(\beta-\alpha)\\
    &\leq \alpha(a-b)\\
    &=a\max(0,\alpha-\beta)+\alpha \max(0,a-b).
\end{align}
Therefore the lemma is proved.
\end{proof}

Now we can prove the following.

\begin{lemma}\label{lem:combined2}
For any $k=0,\dots, K$, we have
\begin{align}
    \sum_{i\in V}\sum_{A_1,\dots, A_k\subseteq V}\max\left(0,\Pr[\mathcal{P}(A_1,\dots, A_k)]-\Pr[\mathcal{P}^i(A_1,\dots, A_k)]\right)\leq 4k\epsilon^{-3}.
\end{align}
\end{lemma}
\begin{proof}
We prove by induction. If $k=0$, then the statement is obvious. If $k>0$, then for any sets $A_1,\dots, A_k\subseteq V$, we have
\begin{align}
    & \max\left(0,\Pr[\mathcal{P}(A_1,\dots, A_k)]-\Pr[\mathcal{P}^i(A_1,\dots, A_k)]\right)\\
    &= \max\left(0,\Pr[\mathcal{P}(A_1,\dots, A_{k-1})]\Pr[A_k=R_k\mid\mathcal{P}(A_1,\dots, A_{k-1})]\right.\nonumber \\
    & \quad \quad \quad \left.-\Pr[\mathcal{P}^i(A_1,\dots, A_{k-1})]\Pr[A_k=R^i_k\mid\mathcal{P}^i(A_1,\dots, A_{k-1})]\right)\\
    & \leq \Pr[A_k=R_k\mid\mathcal{P}(A_1,\dots, A_{k-1})]\nonumber \\
    & \quad \quad \times \max \left(0,\Pr[\mathcal{P}(A_1,\dots, A_{k-1})]-\Pr[\mathcal{P}^i(A_1,\dots, A_{k-1})]\right)\label{eq:sw1}\\
    &+ \Pr[\mathcal{P}(A_1,\dots, A_{k-1})]\nonumber \\
    & \quad \quad \times \max \left(0,\Pr[A_k=R_k\mid\mathcal{P}(A_1,\dots, A_{k-1})]-\Pr[A_k=R^i_k|\mathcal{P}^i(A_1,\dots, A_{k-1})]\right)\label{eq:sw2}.
\end{align}
Here, the inequality is from Lemma~\ref{lem:tech}.
Therefore, we have
\begin{align}
    &\sum_{i\in V}\sum_{A_1,\dots, A_k\subseteq V}\max\left(0,\Pr[\mathcal{P}(A_1,\dots, A_k)]-\Pr[\mathcal{P}^i(A_1,\dots, A_k)]\right)\\
    & \leq \sum_{i\in V}\sum_{A_1,\dots, A_k\subseteq V}\eqref{eq:sw1}+\sum_{i\in V}\sum_{A_1,\dots, A_k\subseteq V}\eqref{eq:sw2}\\
    &\leq \sum_{A_{k}\subseteq V}\Pr[A_k=R_k|\mathcal{P}(A_1,\dots, A_{k-1})]4(k-1)\epsilon^{-3}\nonumber \\
    &\: +\sum_{A_1,\dots, A_{k-1}\subseteq V}\Pr[\mathcal{P}(A_1,\dots, A_{k-1})]4\epsilon^{-3}\\
    &=4(k-1)\epsilon^{-3}+4\epsilon^{-3}=4k\epsilon^{-3},
\end{align}
where the second inequality is from the induction hypothesis and Lemma~\ref{lem:combined1.5} \ynote{something is wrong because we are proving Lemma~\ref{lem:combined2}}\snote{taiouzumi}. Therefore the lemma is proved.
\end{proof}

Now we evaluate the average sensitivity.
Let $\mathcal{A}^i$ be the output distribution of Algorithm~\ref{alg:knapsack} on the instance $V\setminus \{i\}$. For a set $U$ and the weight limit $W$, let $\mathcal{A}_{\mathrm{SMALL}}(U,W)$ be the output distribution of Algorithm~\ref{alg:smallknapsack} on the instance $(U,W)$. \ynote{Strictly speaking, the algorithm SMALL doesn't take $W$.}

\begin{lemma}\label{lem:largesensitivity}
The average sensitivity of Algorithm~\ref{alg:knapsack} is at most $5\epsilon^{-4}$.
\end{lemma}
\begin{proof}
To bound the earth mover's distance, consider transporting probability mass in such a way that the mass of $\mathcal{A}$ with a particular choice of $(R_1,\ldots,R_K)$ and $k$ is transported to that of $\mathcal{A}^i$ with the same $(R_1,\ldots,R_K)$ and $k$.
The remaining mass is transported arbitrarily.
% Inside the case $R_1=R^i_1, \dots, R_K=R^i_K$, we transport probability such a way that the mass of $\mathcal{A}$ and $\mathcal{A}^i$ with the same choice of $k$ corresponds to each other.
Inside this case, we transport probability in the same way as the analysis of Algorithm~\ref{alg:smallknapsack}. \ynote{should be stated better.}
Now, we have
\begin{align}
    &\frac{1}{n}\sum_{i\in V}\EM(\mathcal{A},\mathcal{A}^i)\\
    &\leq \frac{1}{n}\sum_{i\in V}\sum_{A_1,\dots, A_K\subseteq V}\max\left(0,\Pr[\mathcal{P}(A_1,\dots, A_k)]-\Pr[\mathcal{P}^i(A_1,\dots, A_K)]\right)n\nonumber \\
    &+ \frac{1}{n}\sum_{i\in V}\sum_{A_1,\dots, A_K\subseteq V}\sum_{k\in \{0,\dots, K-1\}}\min\left(\Pr[\mathcal{P}(A_1,\dots, A_k)],\Pr[\mathcal{P}^i(A_1,\dots, A_K)]\right)\nonumber \\
    & \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \times \EM(\mathcal{A}_{\mathrm{SMALL}}(U_{k+1},W_k),\mathcal{A}_{\mathrm{SMALL}}(U^i_{k+1},W_k))\\
    &\leq 4K\epsilon^{-3}+\frac{1}{n}\sum_{i\in V}\sum_{A_1,\dots, A_K\subseteq V}\sum_{k\in \{0,\dots, K-1\}}\Pr[\mathcal{P}(A_1,\dots, A_k)](\epsilon^{-1}+1)\\
    &=4K\epsilon^{-3}+K(\epsilon^{-1}+1)\leq 5\epsilon^{-4},
\end{align}
where the first inequality is from our choice of transporting probability mass, the second inequality is from Lemmas~\ref{lem:smallsensitivity} and Lemma~\ref{lem:combined2}, and the last inequality is from $K=\lceil \epsilon^{-1} \rceil$ and $\epsilon\leq 0.01$. Therefore the lemma is proved.
\end{proof}

Therefore we have the following main theorem.

\begin{theorem}\label{thm:main}
For any $\epsilon>0$, the knapsack problem admits $(1-\epsilon)$-approximation algorithm with average sensitivity $O(\epsilon^{-4})$.
\end{theorem}
\begin{proof}
Applying Lemma~\ref{lem:largeapprox} and Lemma~\ref{lem:largesensitivity} by replacing $\epsilon$ by $\min\left(0.01, \frac{\epsilon}{8}\right)$ proves this theorem.
\end{proof}


==> old/small_old.tex <==
%!TEX root=./main.tex

\section{Small Items}\label{sec:small-weight}
In this section, we show a $(1-\epsilon)$-approximation algorithm on instances with all the items having weight at most $\epsilon$.
 % fraction of the weight limit.

We first consider the following greedy algorithm:
Reorder the items in $V$ so that $v(1)/w(1)\geq \cdots \geq v(n)/w(n)$, take the maximum index $t$ with $\sum_{i=1}^{t}w(i)\leq 1$, and then output the set $\{1,\dots, t\}$.
This algorithm is natural and indeed has $(1-\epsilon)$-approximation when every item has weight at most $\epsilon$.
However, the average sensitivity is unbounded:
\begin{proposition}
  The average sensitivity of the greedy algorithm can be arbitrary large even when every item has weight at most $\epsilon$.
\end{proposition}
\begin{proof}
Let $k \geq \lceil \epsilon^{-1} \rceil$ be an integer.
Let $V_1$ be the set of $k$ copies of an item with weight $\frac{1}{k}$ and value $\frac{1}{k}$, $V_2$ be the set of $k$ copies of an item with weight $\frac{1}{k^2}$ and value $\frac{1}{k^3}$, and let $V=V_1\cup V_2$.
The greedy algorithm run on the instance $V$ outputs $V_1$.
Deleting an item in $V_2$ does not change the output.
However, if an item $i\in V_1$ is deleted, the greedy algorithm outputs $V\setminus \{i\}$. Therefore, the average sensitivity is
\begin{align}
    \frac{k}{2k}\cdot 0 + \frac{k}{2k} \cdot (k+1) =\frac{k+1}{2},
\end{align}
which can be arbitrary large.
\end{proof}
The issue of the greedy algorithm is that, if there are many small items ``right after'' the weight limit (e.g., the items in $V_2$ in the instance used in the proof above), deleting an item in the current solution may cause the algorithm to add many of the small items instead.
To resolve this issue, we uniformly sample a weight limit from a distribution from $[1-\epsilon,1]$, instead of fixing it to $1$.
A pseudocode is given in Algorithm~\ref{alg:smallknapsack}.

\begin{algorithm}[t!]
\caption{Less-sensitive knapsack for the weight of all items are at most $\delta$}
\begin{algorithmic}[1]\label{alg:smallknapsack}
\STATE Sort the items of $V$ so that $v(1)/w(1)\geq \cdots \geq v(n)/w(n)$.
\STATE Let $W$ be sampled from $[1-\epsilon,1]$ uniformly at random.
\STATE Let $t$ be the maximum index with $\sum_{i=1}^{t}w(i)\leq W$.\label{line:smalltaket}
\RETURN $\{1,\dots, t\}$.
%\STATE Let $p$ be a variable in $[0,c)$ from uniform distribution
%\STATE Let $a$ be a variable in $[0,1)$ from uniform distribution
%\STATE Let $A=\{j : \sum_{i=1}^{j-1}w_i\not \in [a,a+p\delta)\}$
%\STATE Let $l$ be the maximum index with $\sum_{i\in \{1,\dots, l\}\cap A} w_i \leq 1$
%\RETURN $\{1,\dots, l\}\setminus A$
\end{algorithmic}
\end{algorithm}

First we analyze its approximation ratio. For $W\in [1-\epsilon,1]$, let $S(W)$ (resp., $S^i(W)$) be the output of the greedy algorithm run on $V$ (resp., $V\setminus \{i\}$) when the weight limit is set to $W$.
Note that Algorithm~\ref{alg:smallknapsack} run on $V$ (resp., $S \setminus \{i\}$) outputs $S(W)$ (resp., $S^i(W)$), where $W$ is uniformly sampled from $[1-\epsilon,1]$.
The following lemma is obtained from a standard argument about the knapsack problem.
\begin{lemma}\label{lem:smallapprox}
Algorithm~\ref{alg:smallknapsack} has approximation ratio $1-2\epsilon$.
\end{lemma}
\begin{proof}
Let $S$ be the output of the algorithm. We have
\begin{align}
    \E[v(S)] = \E_W[v(S(W))]\geq \E_W \left[ \int_{0}^{W-\epsilon}\rho(x)\mathrm{d}x\right] \geq \int_{0}^{1-2\epsilon}\rho(x)\mathrm{d}x\geq (1-2\epsilon)\FOPT(V,1)\geq (1-2\epsilon)\OPT(V,1),
\end{align}
where the first inequality is by $\sum_{i=1}^{t}w(i)\geq W-\epsilon$ guaranteed at Line~\ref{line:smalltaket}, the second inequality is by $W\geq 1-\epsilon$, the third inequality is by Lemma~\ref{lem:fracbasic} and the non-increasing property of $\rho$, and the last inequality is by $\FOPT(V,1)\geq \OPT(V,1)$
\end{proof}

Now we analyze average sensitivity.
\begin{lemma}\label{lem:smallsum}
For any $j\in V$, it holds that
\begin{align}
    \int_{1-\epsilon}^{1}\sum_{i\in V}\left|1_{j\in S(W)\triangle S^i(W)}\right|\mathrm{d}W\leq 1+\epsilon.
\end{align}
\end{lemma}
\begin{proof}
Note that, $j\in S(W)$ implies $j\in S^i(W)$ unless $i=j$. Therefore, we have
\begin{align}
    \sum_{i\in V}\left|1_{j\in S(W)\triangle S^i(W)}\right|
    \leq \sum_{i\in V, i\neq j}1_{j\in S^i(W)\setminus S(W)} + 1.\label{eq:removeij}
\end{align}

Suppose $i\neq j$. Then, $j\in S^i(W)\setminus S(W)$ holds if and only if $i\in S(W)$ and $w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})$. Let $k$ be the maximum index such that $w(\{1,\dots, k\})\leq 1$. Then, we have
\begin{align}
    &\int_{1-\epsilon}^{1}\sum_{i\in V}\left|1_{j\in S(W)\triangle S^i(W)}\right|\mathrm{d}W\\
    &\leq \int_{1-\epsilon}^{1}\left(\sum_{i\in V, i\neq j}1_{j\in S^i(W)\setminus S(W)} + 1\right)\mathrm{d}W\\
    &\leq \int_{1-\epsilon}^{1}\sum_{i\in \{1,\dots, k\}}1_{w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})}\mathrm{d}W + \epsilon\\
    &= \sum_{i\in \{1,\dots, k\}}\int_{1-\epsilon}^{1}1_{w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})}\mathrm{d}W + \epsilon\\
    &\leq \sum_{i\in \{1,\dots, k\}}w(i) + \epsilon
     \leq 1 + \epsilon.
\end{align}
Here, the first inequality is by~\eqref{eq:removeij}, the second inequality is the rephrase of the condition $j\in S^i(W)\setminus S(W)$ mentioned above, the third inequality is by $w(\{1,\dots, j\})-w(\{1,\dots, j\}\setminus \{i\}) \leq  w(i)$ and the distribution of $W$, and the last inequality is from the definition of $k$.
\end{proof}

Now we bound average sensitivity.
\begin{lemma}\label{lem:smallsensitivity}
Algorithm~\ref{alg:smallknapsack} has average sensitivity $\epsilon^{-1}+1$.
\end{lemma}
\begin{proof}
Let $\mathcal{A}_{\text{SMALL}}$ (resp., $\mathcal{A}_{\text{SMALL}}^i\;(i \in V)$) be the output distribution of Algorithm~\ref{alg:smallknapsack} run on the instance $V$ (resp., $V\setminus \{i\}$).
For each $i\in V$, we bound the earth mover's distance between $\mathcal{A}_{\text{SMALL}}$ to $\mathcal{A}_{\text{SMALL}}^i$ by transporting the probability mass of $S(W)$ to $S^i(W)$. Now, we have
\begin{align}
    \frac{1}{n}\sum_{i\in V}\EM(\mathcal{A}_{\text{SMALL}},\mathcal{A}_{\text{SMALL}}^i)
    &\leq \frac{1}{n}\sum_{i\in V}\frac{1}{\epsilon}\int_{1-\epsilon}^{1}\sum_{j\in V}\left|1_{j\in S(W)\triangle S^i(W)}\right|\mathrm{d}W\\
    &\leq \frac{1}{n\epsilon}\sum_{j\in V}\left(1+\epsilon\right)
    = \epsilon^{-1}+1,
\end{align}
where the first inequality is from the probability transportation, the second inequality is obtained by swapping sum and integral and applying Lemma~\ref{lem:smallsum}.
\end{proof}



==> small_app.tex <==
%!TEX root=./main.tex

\section{Items with Small Values: Analysis}\label{app:small}

In this section, we prove~\ref{thm:small} by analyzing Algorithm~\ref{alg:smallknapsack}.
As in~\cref{sec:small-weight}, we assume that the weight limit is $1$ (and use the symbol $W$ for a different purpose).


\subsection{Modified Greedy Algorithm}\label{sec:greedy}
We first consider the following greedy algorithm:
Reorder the items in $V$ in a non-increasing order of efficiency, i.e., $v(1)/w(1)\geq \cdots \geq v(n)/w(n)$, take the maximum index $t$ with $\sum_{i=1}^{t}w(i)\leq 1$, and then output the set $\{1,\dots, t\}$.
It is easy to verify that this natural algorithm outputs a solution with value at least $\OPT(V)-\delta$ when every item has value at most $\delta$.
However, its average sensitivity is unbounded.
To confirm this, we consider the proof of Proposition~\ref{prop:unbounded}.
\begin{proof}[Proof of Proposition~\ref{prop:unbounded}]
%Let $k \geq \lceil \delta^{-1} \rceil$ be an integer.
Let $k$ be an integer.
Let $V_1$ be the set of $k$ copies of an item with weight $\frac{1}{k}$ and value $\frac{1}{k}$, $V_2$ be the set of $k$ copies of an item with weight $\frac{1}{k^2}$ and value $\frac{1}{k^3}$, and let $V=V_1\cup V_2$.
The optimal solution for the instance $V$ is $V_1$, which does not change upon deleting an item in $V_2$.
%The greedy algorithm run on the instance $V$ outputs $V_1$.
%Deleting an item in $V_2$ does not change the output.
However, if an item $i\in V_1$ is deleted, the optimal solution changes to $V\setminus \{i\}$. Therefore, the average sensitivity is
\[
    \frac{k}{2k}\cdot 0 + \frac{k}{2k} \cdot (k+1) =\frac{k+1}{2},
\]
which is as large as $\Omega(n)$.
% \ynote{The argument is the same as the one presented in the introduction. Can we merge them?}\snote{merged}
\end{proof}
This proof also shows that for any $\delta>0$, the natural greedy algorithm has an unbounded average sensitivity even if the values of items are at most $\delta$, by setting $k\geq \lceil \delta^{-1} \rceil$.
%We can observe that the optimal solutions of the instance and the instance with an item deleted coincide with the outputs of the greedy algorithm on the respective instances.

An issue of the greedy algorithm is that, when there are many small items (in weight) ``right after'' the weight limit in the efficiency ordering (e.g., the items in $V_2$ in the instance used in the proof of Proposition~\ref{prop:unbounded}), deleting an item in the current solution may cause the algorithm to add many of the small items.
To resolve this issue, we uniformly sample the weight limit $W$ from $[1-\epsilon,1]$, instead of fixing it to $1$.


\subsection{Analysis}
First we analyze the approximation ratio of Algorithm~\ref{alg:smallknapsack}.
For $W\in [1-\epsilon,1]$, let $S(W)$ (resp., $S^i(W)$) be the output of the greedy algorithm run on $V$ (resp., $V\setminus \{i\}$) with the weight limit set to $W$.
Note that Algorithm~\ref{alg:smallknapsack} run on $V$ (resp., $V \setminus \{i\}$) first samples $W$ from $[1-\epsilon,1]$ uniformly at random and then outputs $S(W)$ (resp., $S^i(W)$).
The following lemma is obtained from a standard argument about the knapsack problem.
\begin{lemma}\label{lem:smallapprox}
Suppose every item has value at most $\delta$.
Then, Algorithm~\ref{alg:smallknapsack} outputs a solution with value at least $(1-\epsilon)\FOPT(V)-\delta$.
\end{lemma}
\begin{proof}
We have
\[
    \sum_{i=1}^{t}w(i)\geq \FOPT(V,W)-\delta \geq W\FOPT(V,1)-\delta \geq (1-\epsilon)\FOPT(V,1)-\delta,    
\]
where the first inequality is from Lemma~\ref{lem:fractional-optimal-solution}, the second inequality is from Lemma~\ref{lem:frac_efficient}, and the last inequality is from $W\geq 1-\epsilon$.
\end{proof}

We turn to analyzing the average sensitivity of Algorithm~\ref{alg:smallknapsack}.
We start by proving the following auxiliary lemma.
\begin{lemma}\label{lem:smallsum}
For any $j\in V$, it holds that
\[
    \int_{1-\epsilon}^{1}\sum_{i\in V} 1_{j\in S(W)\triangle S^i(W)}\mathrm{d}W\leq 1+\epsilon.
\]
\end{lemma}
\begin{proof}
Note that, $j\in S(W)$ implies $j\in S^i(W)$ unless $i=j$. Therefore, we have
\begin{align}
    \sum_{i\in V} 1_{j\in S(W)\triangle S^i(W)}
    \leq \sum_{i\in V, i\neq j}1_{j\in S^i(W)\setminus S(W)} + 1.\label{eq:removeij}
\end{align}

Suppose $i\neq j$. Then, $j\in S^i(W)\setminus S(W)$ holds if and only if $i\in S(W)$ and $w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})$. Let $k$ be the largest index such that $w(\{1,\dots, k\})\leq 1$. Then, we have
\begin{align*}
    &\int_{1-\epsilon}^{1}\sum_{i\in V}1_{j\in S(W)\triangle S^i(W)}\mathrm{d}W
    \leq \int_{1-\epsilon}^{1}\left(\sum_{i\in V, i\neq j}1_{j\in S^i(W)\setminus S(W)} + 1\right)\mathrm{d}W\\
    &\leq \int_{1-\epsilon}^{1}\sum_{i = 1}^k 1_{w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})}\mathrm{d}W + \epsilon
    = \sum_{i = 1}^k\int_{1-\epsilon}^{1}1_{w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})}\mathrm{d}W + \epsilon\\
    &\leq \sum_{i = 1}^k w(i) + \epsilon
     \leq 1 + \epsilon.
\end{align*}
Here, the first inequality is given by~\eqref{eq:removeij}, the second inequality is due to the rephrase of the condition $j\in S^i(W)\setminus S(W)$ mentioned above, the third inequality is by $w(\{1,\dots, j\})-w(\{1,\dots, j\}\setminus \{i\}) \leq  w(i)$ and the distribution of $W$, and the last inequality arises from the definition of $k$.
\end{proof}

Let $\mathcal{A}_{\text{SMALL}}$ (resp., $\mathcal{A}_{\text{SMALL}}^i\;(i \in V)$) be the output distribution of Algorithm~\ref{alg:smallknapsack} run on the instance $V$ (resp., $V\setminus \{i\}$). Now, we show the following:
\begin{lemma}\label{lem:smallsensitivity}
Algorithm~\ref{alg:smallknapsack} has average sensitivity $\epsilon^{-1}+1$.
\end{lemma}
\begin{proof}
For each $i\in V$, we bound the earth mover's distance between $\mathcal{A}_{\text{SMALL}}$ to $\mathcal{A}_{\text{SMALL}}^i$ by transporting the maximum possible probability mass of $S(W)$ to $S^i(W)$. Now, we have
\begin{align*}
    \frac{1}{n}\sum_{i\in V}\EM(\mathcal{A}_{\text{SMALL}},\mathcal{A}_{\text{SMALL}}^i)
    &\leq \frac{1}{n}\sum_{i\in V}\left(\frac{1}{\epsilon}\int_{1-\epsilon}^{1}\left(\sum_{j\in V} 1_{j\in S(W)\triangle S^i(W)}\right)\mathrm{d}W\right)\\
    &\leq \frac{1}{n\epsilon}\sum_{j\in V}\left(1+\epsilon\right)
    = \epsilon^{-1}+1,
\end{align*}
where the first inequality arises from the transport of the probability mass and the definition of $W$ in Algorithm~\ref{alg:smallknapsack}, and the second inequality is obtained by swapping the sum and integral and applying Lemma~\ref{lem:smallsum}.
\end{proof}
Theorem~\ref{thm:small} is immediate by Lemmas~\ref{lem:smallapprox} and~\ref{lem:smallsensitivity}.




==> small_new.tex <==
%!TEX root=./main.tex

\section{Items with Small Values}\label{sec:small-weight}

In this section, we provide a stable-on-average algorithm for instances with each item having a small value.
Specifically, we show the following:
\begin{theorem}\label{thm:small}
    For any $\epsilon,\delta > 0$, there exists an algorithm for the knapsack problem with average sensitivity $O(\epsilon^{-1})$ that, given an instance $(V,W)$ with each item having value at most $\delta$, outputs a solution with value at least $(1-\epsilon)\FOPT(V,W)-\delta$.
\end{theorem}
This algorithm will be used in our algorithm for the general case as a subroutine in Section~\ref{sec:general}.
Note that it suffices to design an algorithm for the case in which the weight limit is $1$ because we can first divide the weight of each item by $W$ and feed the resulting instance to the algorithm.
Hence in the following discussion, we assume that the weight limit is $1$ (and use the symbol $W$ for a different purpose).


\subsection{Modified Greedy Algorithm}\label{sec:greedy}
We first consider the following greedy algorithm:
Reorder the items in $V$ in a non-increasing order of efficiency, i.e., $v(1)/w(1)\geq \cdots \geq v(n)/w(n)$, take the maximum index $t$ with $\sum_{i=1}^{t}w(i)\leq 1$, and then output the set $\{1,\dots, t\}$.
It is easy to verify that this natural algorithm outputs a solution with value at least $\OPT(V)-\delta$ when every item has value at most $\delta$.
However, its average sensitivity is unbounded.
To confirm this, we consider the proof of Proposition~\ref{prop:unbounded}.
\begin{proof}[Proof of Proposition~\ref{prop:unbounded}]
%Let $k \geq \lceil \delta^{-1} \rceil$ be an integer.
Let $k$ be an integer.
Let $V_1$ be the set of $k$ copies of an item with weight $\frac{1}{k}$ and value $\frac{1}{k}$, $V_2$ be the set of $k$ copies of an item with weight $\frac{1}{k^2}$ and value $\frac{1}{k^3}$, and let $V=V_1\cup V_2$.
The optimal solution for the instance $V$ is $V_1$, which does not change upon deleting an item in $V_2$.
%The greedy algorithm run on the instance $V$ outputs $V_1$.
%Deleting an item in $V_2$ does not change the output.
However, if an item $i\in V_1$ is deleted, the optimal solution changes to $V\setminus \{i\}$. Therefore, the average sensitivity is
\[
    \frac{k}{2k}\cdot 0 + \frac{k}{2k} \cdot (k+1) =\frac{k+1}{2},
\]
which is as large as $\Omega(n)$.
% \ynote{The argument is the same as the one presented in the introduction. Can we merge them?}\snote{merged}
\end{proof}
This proof also shows that for any $\delta>0$, the natural greedy algorithm has an unbounded average sensitivity even if the values of items are at most $\delta$, by setting $k\geq \lceil \delta^{-1} \rceil$.
%We can observe that the optimal solutions of the instance and the instance with an item deleted coincide with the outputs of the greedy algorithm on the respective instances.

An issue of the greedy algorithm is that, when there are many small items (in weight) ``right after'' the weight limit in the efficiency ordering (e.g., the items in $V_2$ in the instance used in the proof of Proposition~\ref{prop:unbounded}), deleting an item in the current solution may cause the algorithm to add many of the small items.
To resolve this issue, we uniformly sample the weight limit $W$ from $[1-\epsilon,1]$, instead of fixing it to $1$.
A pseudocode of our modified greedy algorithm is given in Algorithm~\ref{alg:smallknapsack}.

\begin{algorithm}[t!]
\caption{A $(1-O(\epsilon))$-approximation algorithm with small average sensitivity}\label{alg:smallknapsack}
% \begin{algorithmic}[1]
% \Procedure{\emph{\Call{ModifiedGreedy}{$\epsilon,V,W$}}}{
%     Run \Call{ModifiedGreedy'}{$\epsilon,V$} after replacing $w(i)$ with $w(i)/W$ for every $i \in V$.
% }
\Procedure{\emph{\Call{ModifiedGreedy}{$\epsilon,V$}}}{
    Reorder the items of $V$ so that $v(1)/w(1)\geq \cdots \geq v(n)/w(n)$\;
    Let $W$ be sampled from $[1-\epsilon,1]$ uniformly at random\;
    Let $t$ be the maximum index with $\sum_{i=1}^{t}w(i)\leq W$\;\label{line:smalltaket}
    \Return $\{1,\dots, t\}$.
}
%\STATE Let $p$ be a variable in $[0,c)$ from uniform distribution
%\STATE Let $a$ be a variable in $[0,1)$ from uniform distribution
%\STATE Let $A=\{j : \sum_{i=1}^{j-1}w_i\not \in [a,a+p\delta)\}$
%\STATE Let $l$ be the maximum index with $\sum_{i\in \{1,\dots, l\}\cap A} w_i \leq 1$
%\RETURN $\{1,\dots, l\}\setminus A$
% \end{algorithmic}
\end{algorithm}

\subsection{Analysis}
First we analyze the approximation ratio of Algorithm~\ref{alg:smallknapsack}.
For $W\in [1-\epsilon,1]$, let $S(W)$ (resp., $S^i(W)$) be the output of the greedy algorithm run on $V$ (resp., $V\setminus \{i\}$) with the weight limit set to $W$.
Note that Algorithm~\ref{alg:smallknapsack} run on $V$ (resp., $V \setminus \{i\}$) first samples $W$ from $[1-\epsilon,1]$ uniformly at random and then outputs $S(W)$ (resp., $S^i(W)$).
The following lemma is obtained from a standard argument about the knapsack problem.
\begin{lemma}\label{lem:smallapprox}
Suppose every item has value at most $\delta$.
Then, Algorithm~\ref{alg:smallknapsack} outputs a solution with value at least $(1-\epsilon)\FOPT(V)-\delta$.
\end{lemma}
\begin{proof}
We have
\[
    \sum_{i=1}^{t}w(i)\geq \FOPT(V,W)-\delta \geq W\FOPT(V,1)-\delta \geq (1-\epsilon)\FOPT(V,1)-\delta,    
\]
where the first inequality is from Lemma~\ref{lem:fractional-optimal-solution}, the second inequality is from Lemma~\ref{lem:frac_efficient}, and the last inequality is from $W\geq 1-\epsilon$.
\end{proof}

We turn to analyzing the average sensitivity of Algorithm~\ref{alg:smallknapsack}.
We start by proving the following auxiliary lemma.
\begin{lemma}\label{lem:smallsum}
For any $j\in V$, it holds that
\[
    \int_{1-\epsilon}^{1}\sum_{i\in V} 1_{j\in S(W)\triangle S^i(W)}\mathrm{d}W\leq 1+\epsilon.
\]
\end{lemma}
\begin{proof}
Note that, $j\in S(W)$ implies $j\in S^i(W)$ unless $i=j$. Therefore, we have
\begin{align}
    \sum_{i\in V} 1_{j\in S(W)\triangle S^i(W)}
    \leq \sum_{i\in V, i\neq j}1_{j\in S^i(W)\setminus S(W)} + 1.\label{eq:removeij}
\end{align}

Suppose $i\neq j$. Then, $j\in S^i(W)\setminus S(W)$ holds if and only if $i\in S(W)$ and $w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})$. Let $k$ be the largest index such that $w(\{1,\dots, k\})\leq 1$. Then, we have
\begin{align*}
    &\int_{1-\epsilon}^{1}\sum_{i\in V}1_{j\in S(W)\triangle S^i(W)}\mathrm{d}W
    \leq \int_{1-\epsilon}^{1}\left(\sum_{i\in V, i\neq j}1_{j\in S^i(W)\setminus S(W)} + 1\right)\mathrm{d}W\\
    &\leq \int_{1-\epsilon}^{1}\sum_{i = 1}^k 1_{w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})}\mathrm{d}W + \epsilon
    = \sum_{i = 1}^k\int_{1-\epsilon}^{1}1_{w(\{1,\dots, j\}\setminus \{i\}) \leq W < w(\{1,\dots, j\})}\mathrm{d}W + \epsilon\\
    &\leq \sum_{i = 1}^k w(i) + \epsilon
     \leq 1 + \epsilon.
\end{align*}
Here, the first inequality is given by~\eqref{eq:removeij}, the second inequality is due to the rephrase of the condition $j\in S^i(W)\setminus S(W)$ mentioned above, the third inequality is by $w(\{1,\dots, j\})-w(\{1,\dots, j\}\setminus \{i\}) \leq  w(i)$ and the distribution of $W$, and the last inequality arises from the definition of $k$.
\end{proof}

Let $\mathcal{A}_{\text{SMALL}}$ (resp., $\mathcal{A}_{\text{SMALL}}^i\;(i \in V)$) be the output distribution of Algorithm~\ref{alg:smallknapsack} run on the instance $V$ (resp., $V\setminus \{i\}$). Now, we show the following:
\begin{lemma}\label{lem:smallsensitivity}
Algorithm~\ref{alg:smallknapsack} has average sensitivity $\epsilon^{-1}+1$.
\end{lemma}
\begin{proof}
For each $i\in V$, we bound the earth mover's distance between $\mathcal{A}_{\text{SMALL}}$ to $\mathcal{A}_{\text{SMALL}}^i$ by transporting the maximum possible probability mass of $S(W)$ to $S^i(W)$. Now, we have
\begin{align*}
    \frac{1}{n}\sum_{i\in V}\EM(\mathcal{A}_{\text{SMALL}},\mathcal{A}_{\text{SMALL}}^i)
    &\leq \frac{1}{n}\sum_{i\in V}\left(\frac{1}{\epsilon}\int_{1-\epsilon}^{1}\left(\sum_{j\in V} 1_{j\in S(W)\triangle S^i(W)}\right)\mathrm{d}W\right)\\
    &\leq \frac{1}{n\epsilon}\sum_{j\in V}\left(1+\epsilon\right)
    = \epsilon^{-1}+1,
\end{align*}
where the first inequality arises from the transport of the probability mass and the definition of $W$ in Algorithm~\ref{alg:smallknapsack}, and the second inequality is obtained by swapping the sum and integral and applying Lemma~\ref{lem:smallsum}.
\end{proof}
Theorem~\ref{thm:small} is immediate by Lemmas~\ref{lem:smallapprox} and~\ref{lem:smallsensitivity}.



